Lessons Learned on MPI+Threads Communication

Hybrid MPI+threads programming is gaining prominence, but, in practice, applications perform slower with it compared to the MPI everywhere model. The most critical challenge to the parallel efficiency of MPI+threads applications is slow MPI_THREAD_MULTIPLE performance. MPI libraries have recently made significant strides on this front, but to exploit their capabilities, users must expose the communication parallelism in their MPI+threads applications. Recent studies show that MPI 4.0 provides users with new performance-oriented options to do so, but our evaluation of these new mechanisms shows that they pose several challenges. An alternative design is MPI Endpoints. In this paper, we present a comparison of the different designs from the perspective of MPI's end-users: domain scientists and application developers. We evaluate the mechanisms on metrics beyond performance such as usability, scope, and portability. Based on the lessons learned, we make a case for a future direction.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> text/accel_discussion.tex <==
\section{Discussion in the context of accelerators}
\label{sec:heterogenous_computing}

\threads{} is a critical model to program
the many-core processors of the current
HPC clusters and the upcoming exascale
systems. It is imperative that applications
perform productively with it. The key
to achieving high performance with
\threads{} requires efforts from both
MPI library developers and application
developers. Recently, MPI libraries have
made significant strides in this regard,
and now the ball is in the court of
domain scientists to expose 
communication parallelism to utilize the
new fast \threads{} libraries. Domain
scientists, however, face many programming challenges
with the current direction that the MPI
community is pursuing with respect
to the mechanisms of exposing
communication independence between
threads.
\changed{
The limitations of existing MPI
mechanisms and partitioned communication imply
that the fraction of
\threads{} applications achieving
high performance will grow at a
slow rate. Our qualitative analysis in this paper,
backed by direct collaborations with
MPI's end users from a variety of domains,
shows that the alternative design of MPI Rankpoints
is a seamless option. MPI
Rankpoints has already been deliberated by
the MPI Forum (in the form of MPI Endpoints)
and the challenge with \emph{rankpoints} lies not
with the applicability of the mechanism to \threads{} applications
but with its formal approval to be introduced
into the standard. We encourage the MPI Forum
and the MPI community to consider the
perspective of MPI's end-users, the domain
scientists, as opposed to only performance
while debating the different interfaces.
}

==> text/background.tex <==
\section{Background}
\label{sec:background}

\subsection{Why hybrid \threads{}?}
\label{sec:why_mpi_threads}

The Message Passing Interface (MPI)  is the
defacto standard for programming supercomputing
applications. The traditional way to use it has been
the \everywhere{} (a process per core) approach
where a domain scientist, MPI's end user, spawns as
many processes as there are cores 
to transparently utilize both the core-level and
node-level parallelism. The \everywhere{} model
has served the community well for decades, but
given the architecture trends of modern systems,
domain scientists are no longer able to scale their
applications with \everywhere{}. The reason is
two fold: first, the number of cores has increased
disproportionately to the growth in other on-node
resources such as memory, TLB space, and network
resources (work queues and doorbell registers) over the last decade~\cite{fugaku,thakur2010mpi};
second, the memory requirements of \everywhere{}
increase with the number of cores per node~\cite{rabenseifner2009hybrid}.
Coupled together, these two reasons have caused
applications to run out of memory on large domains
with \everywhere{}~\cite{pall2014tackling, bulucc2017distributed}.
Features such as MPI Shared Memory~\cite{hoefler2013mpi+}
alleviate the wastage problem, but they address sharing
only a subset of the resources. MPI Shared Memory does
not reduce TLB pressure in the manner that \threads{}
does. Hence, it is not a generic solution for all on-node resources.
More generally, the static split of resources between
processes in \everywhere{} leads to high resource
wastage (\eg{}, 94\% wastage of
network resources~\cite{zambre2018scalable}).

To program modern processors in a scalable fashion,
domain scientists have introduced a ``new normal''
in their programming model of choice: \threads{}
(\eg{}, MPI+OpenMP). \threads{} allows applications
to utilize the many cores with threads and efficiently
share the limited on-node resources between cores with a single process
per node (or NUMA domain). With this approach, applications
are able to scale to much larger domain sizes on modern
systems.

\subsection{Why \threads{} communication matters?}
\label{sec:what_about_mpi_threads_comm}

Although applications can efficiently scale with \threads{}, in practice, they
tend to perform slower than their \everywhere{}
counterparts~\cite{jin2011high,bulucc2017distributed,higgins2015hybrid, pall2014tackling}. The reason is that
\threads{} programming raises new
challenges, such as mitigating thread-synchronization
overheads~\cite{hetland2019paths,rodchenko2015effective, iwainsky2015many},
and preventing performance-degrading memory
accesses (\eg{}, false sharing), that are not present in
\everywhere{}. The most critical challenge, however, is the
dismal communication performance of an \threads{}
application~\cite{zambre2021logically,amer2015mpi+,thakur2010mpi,amer2019software,balaji2010fine}.
\changed{
This challenge is a pressing bottleneck because most scientific
simulation campaigns run close to the strong-scaling limit
where communication occupies a significant portion of the
application's
runtime~\cite{raffenetti2017mpi,sahasrabudhe2020improving,wang2020pencil,wang2021algorithm}.
}

\changed{
Furthermore, as an application approaches the strong-scaling
limit, the size of each individual message decreases, and the
communication performance is limited by the rate of
issuing a message rather than the network bandwidth.
In this paradigm, the interoperability of
threads with MPI is critical for the performance of an \threads{}
application.} MPI defines multiple levels of threading support
going from a highly restrictive level---only one thread will
execute---to a completely flexible level: multiple threads can execute
MPI operations in parallel (\ie, \multiple). According
to a 2017 survey of applications chosen as candidates for the
upcoming exascale systems, domain scientists prefer
using the flexible \multiple{} level but do not do so currently
primarily because of poor performance~\cite{bernholdt2020survey}.
\changed{
Developers of modern distributed deep learning frameworks
share the same experience too~\cite{daily2018gossipgrad,tensorflow}.
}

\subsection{Why has \threads{} communication been slow?}

The poor performance is more than just an engineering problem.
It also stems from an outdated view
held by the supercomputing community: \emph{the network is
a single device}. Modern network hardware features
multiple dimensions of parallelism (multiple hardware queues
per NIC and multiple NICs per node), but
both MPI libraries and domain scientists do not
capitalize on the underlying network parallelism since all
operations from a process funnel through a single
network queue.

By default, the MPI standard enforces certain ordering
constraints for determinism. But it also provides certain
mechanisms (\eg, communicators) to
overcome its ordering constraints. Most production MPI
libraries today, however, conservatively maintain MPI's ordering
constraints by utilizing only a single network hardware
queue. Only recently (starting in 2019) have MPI libraries
made significant strides in achieving scalable \multiple{}
performance that matches that of \everywhere{}.
A key factor in this improved performance is
the MPI library's ability to map \emph{logically parallel
communication}---operations that are not ordered
according to MPI's semantics---to the underlying network
parallelism~\cite{zambre2020learned, patinyasakdikul2019give}.
Domain scientists, however, typically do not expose such
logically parallel communication in their applications.
The reason is not only the outdated view, but also
that existing MPI semantics can prevent
the exposure of all of the communication
independence between threads especially in irregular
communication patterns.

==> text/coll_communication.tex <==
\section{Comparison of Designs for Collective Operations}
\label{sec:conversations}

\subsection{Collective}

Research efforts with respect to implementing
collectives in a hybrid \threads{} environment
have primarily revolved around hierarchical
algorithms where threads first implement the
collective (\eg{}, allreduce) amongst themselves
and then one thread on each node participates
in the internode collective~\cite{li2013numa,zhou2020collectives}.
Recent studies using a fast \threads{} library (Intel
MPI 2019~\cite{intelmpi}), however, demonstrate performance
benefits when multiple threads drive a collective
in parallel~\cite{wende2019openmp,boyle2017accelerating}.
Although existing MPI semantics do not allow multiple
threads to participate in the collective of a single
communicator, applications may partition the
collective-data of a process across threads and issue
parallel collectives on the different segments of the
data using a distinct communicator for each
thread.

\begin{concern}
	\emph{Concern:} Does that mean  I need to
	handle the intranode portion of a collective?
\end{concern}

%=================================================================
\begin{figure*}[!b]
	\begin{center}
		\includegraphics[width=0.85\textwidth]{pics/collective_mechanisms_comparison.pdf}
	\end{center}
	%	\vspace{-0.5em}
	\caption{Existing mechanisms vs. user-visible endpoints for collective
		communication.}
	\label{fig:collective_compare}
	%	\vspace{-0.5em}
\end{figure*}
%=================================================================

\miniminititle{Existing MPI mechanisms require manual
intra-node collective.}
With existing MPI mechanisms, users need to perform
the intranode portion of the collective (see
\figref{fig:collective_compare}). For example, in an
allreduce collective, the user needs to perform
a reduction step after all threads have completed the
internode part of the allreduce. With user-visible endpoints,
on the other hand, the collective is only one step---all
threads participate
in a collective of the same communicator through
different endpoints. The MPI library then
conducts both the internode and intranode part of
the collective before returning from the operation.
Although the performances of the
two approaches is yet to be compared, we note that, from a
design perspective, the endpoints
approach is better because it does not force the
user to manually handle the intranode portion of
a collective. Arguably, shared-memory
programming models feature direct support for
collectives between threads; for example,
OpenMP supports a reduction operation through
compiler directives. But such support does not
apply to all types of
collective communication that MPI features
(\eg{}, \texttt{MPI\_Alltoall}).
A \naive{} implementation for such cases is likely
to hurt performance for high thread counts (relevant
on existing and upcoming many-core processors).
Efficiently implementing a collective
is not a trivial task; for many years, researchers
have spent numerous efforts into optimizing
collectives~\cite{hoefler2014energy,chan2007collective}.
Manually implementing
tree-style and bucket algorithms is a tedious task that
could instead be handled by the MPI library as is the case
in the user-visible endpoints design.

\miniminititle{Duplicated destination buffers on
	a node with endpoints.}
The interface of user-visible endpoints
results in duplication of data per node in cases
where the result of the collective is the
same across all ranks participating in the operation
(\eg{}, allreduce, broadcast, etc.). The destination
buffers of the endpoints on a single process 
contain the same values (like \everywhere{} where
each process features a copy of the resulting buffer)
when only one such buffer
is needed since all threads can directly read from the
single buffer. With communicators, on the other hand, such
duplication does not exist since the user can perform,
for example, an intra-node reduction
into a single buffer that all threads can read from.
In this regards, the partitioned communication
interface overcomes the duplication issue with
endpoints .
Each partition of a partitioned collective would
be different sections of the input buffer. With
threads driving distinct partitions,
the MPI library would implement both the intranode
and internode portion of a collective, and each process
would host only one buffer that contains the result
of the collective. We note, however, that a case where an \everywhere{} application
has run out of memory solely because of duplication
of a collective's resulting data has not been
demonstrated yet. Hence, the duplication
of data in collectives with user-visible endpoints is not
as concerning as the duplication of domain-level
data that has caused applications to run out of memory
with \everywhere{}. Furthermore, the duplication
does not hold for collectives where the result of the
collective is different for different ranks (\eg{}, alltoall).

%\subsection{Miscellaneous}
%
%Concern: Majority of the effort is in the conversion from MPI everywhere to MPI+threads.
%Is the productivity concern substantial?

==> text/p2p_communication.tex <==
\section{Comparison of Designs for Point-to-point Operations}
\label{sec:conversations}

In this section, we compare how the different
designs (see \secref{sec:schools})
compare against each other with respect to two key metrics:
ease of use (which measures the productivity of domain
scientists), and applicability to different MPI operations (which
measures the scope of the designs). We organize our discussion
by the different types of MPI operations and share
the concerns of end users in each.
\changed{
Given the theoretical
limitations of partitioned operations, we focus our discussion
on existing MPI objects and user-visible endpoints;
we discuss partitioned communication where relevant.
}

\subsection{Point-to-point}


\subsubsection{Mechanism 1: Communicators}
%\minititle{Mechanism 1: Communicators.}
Using distinct communicators is the most explicit
way to express logically parallel communication
for point-to-point operations with MPI's default
semantics (see \secref{sec:existing_mechanisms}).
During our interactions with application developers from
University of Utah (stencil communication in the
hypre linear solver used by Uintah~\cite{sahasrabudhe2020improving}), 
Maison de la Simulation (stencil communication
in Smilei~\cite{derouillat2018smilei}), Pacific Northwest
National Laboratory (graph communication in Vite~\cite{ghosh2018scalable}),
and University of California, Irvine (stencil communication
in Pencil~\cite{wang2020pencil})  we discovered
that the need to \emph{match communicators} makes
exposing logical parallelism between
threads a challenging task. 

\begin{concern}
	\emph{Concern:} Exposing logical
	communication parallelism with communicators is a nightmare!
\end{concern}

Deriving the mathematical relationships of mapping
communicators to threads while ensuring that both the sending
and receiving threads use the same communicator is not
straightforward. This complexity increases with 
the increase in dimensionality and is heightened by the constraint of
using the least possible number of communicators.
This constraint is important since the
number of network hardware contexts is limited~\cite{zambre2018scalable}
(\eg{}, the Intel HFI adapter of the Intel Omni-Path
interconnect features only 160 contexts~\cite{hfi_guide}). By creating more
communicators than there are network resources,
multiple communicators would collide on the same network
resource and serialize communication underneath
even with fully exposed logically parallel communication.

%=================================================================
\begin{figure}[htbp]
	%\centering
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\includegraphics[width=0.5\textwidth]{pics/2d_9pt_stencil_comm_example.pdf}
		%		\vspace{-0.5em}
		\caption{Ideal communicator usage for a 2D 9-point stencil.
			Each box represents a process with 9 threads. Each thread
			has 1 patch. Each color-shape combination represents a
			communicator. Numbers represent thread IDs.}
		\label{fig:2d_stencil_comm}
	\end{minipage}
	\begin{minipage}[t]{0.49\textwidth}
		\centering
		\includegraphics[width=0.6\textwidth]{pics/legion_pattern.pdf}
		%\vspace{-0.5em}
		\caption{Communicator vs. Endpoints for Legion's runtime that
			implements an event-based system using
			multithreaded point-to-point communication. Multiple task threads
			initiate active messages and a polling thread processes the
			incoming events.}
		\label{fig:legion_comm}
	\end{minipage}
	%	\vspace{-1em}
\end{figure}
%=================================================================

\miniminititle{Exposing parallelism with communicators is complex.}
Consider a static (communication pattern of each thread is
fixed) 2D 9-point stencil. \figref{fig:2d_stencil_comm}
shows the ideal communicator usage---minimum number of
communicators with all of the available parallelism exposed---for
such a communication pattern. For a given direction
of communication, we have as many communicators as there 
are communicating threads on the edge (a plane in 3D) since
the operations of the threads are independent. The threads
on a corner, however, use a single communicator for all directions
since their operations for the different directions occur serially.
The mapping of communicators to threads is not
the same on each process. For example, thread 7 of the bottom-left
process in \figref{fig:2d_stencil_comm} must use a communicator
for its north-south communication that is different from the
communicator that thread 7 on the top-left rank uses for the
same north-south direction. This difference in communicators
prevent threads 1 and 7 on a process from using the
same communicator and serializing their communication. In
other words, given a map of communicators for the threads of
a given process, the map for other processes can be derived
by mirroring the map along the change in cartesian coordinates
of the process. Doing so with a logical relation that is programmable
is a hard task.

\miniminititle{Exposing parallelism with communicators is not intuitive.}
To elaborate on this point, we will continue to use the stencil communication
pattern example. The first approach that multiple application developers
(those of Uintah, Smilei and Pencil) thought of using
did not expose all of the available parallelism.
In the 2D example, their intuition
was to create as many communicators as there are threads and
then use communicator $i$ for thread $i$'s send operations and
communicator $j$ for thread $i$'s receive operations where $j$ is
the thread id of the remote thread that thread $i$ is receiving from.
This usage of communicators is correct, but it exposes only half
of the available parallelism. The communication of adjacent threads
on an edge occur in parallel
but the operations of threads on opposite edges use the
same communicator. For example, in \figref{fig:2d_stencil_comm},
thread 1's send operation uses communicator 1, which 
thread 7 also uses for its receive operations. 

\miniminititle{Mismatch in expected mapping to the underlying
	network parallelism due to \changed{high resource requirements.}}
Even if the domain scientist achieves the ideal communicator
usage, the number of communicators required on today's
many-core architectures can be much higher than the number
of underlying network resources. The communication pattern
in real-world stencil applications is typically that of a 3D 27-point
stencil (\eg{}, hypre). Such applications decompose their
domain into cubical patches. If we consider $[x,y,z]$ to be a
vector representing the cubic arrangement of threads in an MPI
process, the least number of communicators we need to express
all of the available logical communication parallelism is
\(
2xy + 2yz + 2xz +
8(xy+ yz + xz - 1) +
4(xz + yz - z) + 4(xy + yz - y)  + 4(xy + xz - x)
\).
The first three terms represent the directions
perpendicular to the 6 faces, the fourth term represents
the 8 corner diagonals, and the last three terms
represent the edge diagonals. If we consider a cluster
that is interconnected with the Intel OPA interconnect
and each node hosts a Intel Knights Landing processor
(\eg{}, the Bebop HPC system at Argonne National
Laboratory), the ideal number of communicators is
808 (1 process per node with $[4,4,4]$ threads per
process), which is over 5$\times$ that of the number
of network hardware resources (160). \changed{In such a scenario,
the domain scientist is expressing all of the available
logical communication parallelism and the application is
using all of the network resources. However, the observed
performance benefit may not be as expected because of
contention on the limited number of network resources,
and the overheads of synchronizing threads when they share
the same network resource.
}

\changed{\miniminititle{Mismatch in expected mapping to the underlying
	network parallelism due to overloaded definitions.}}
Domain scientists typically do not think of communicators as
a means to express communication parallelism. Communicators
are historically viewed as groups of processes or as a
means to isolate matching of messages. That
it can double up as a means to express parallelism
is a corollary of its definition. The
multiple purposes of a communicator can lead to a
mismatch in expected mapping to the underlying network
parallelism. For example, an application can create a set
of communicators for the purposes of grouping different
processes and later use communicators to express
parallelism. The MPI library underneath cannot differentiate
between the two and could end up allocating the underlying
network resources to the communicators used for grouping
different sets of processes, leaving fewer network resources
to map to for logical-parallelism-oriented communicators.
MPI libraries can prevent the second type of mismatch in
expected mapping by introducing  hints that allow an
application to inform the library when it is creating
communicators for the purposes of expressing logically
parallel communication. But such hints would be
implementation-specific.

\miniminititle{Limiting semantics for irregular and dynamic
	communication patterns.}
The root cause of this limitation is that communicators
constrain the task of expressing parallelism with matching
semantics. So, if an application is to express parallelism
with communicators, it must ensure that the sending and
receiving threads use the same communicator. This
matching constraint can be limiting for applications with
dynamic communication patterns where the
communication neighborhood of a thread can change over
time (\eg{}, graph and adaptive mesh refinement applications),
and for applications with irregular communication
patterns where threads are forced to use the same
communicator. \figref{fig:legion_comm} portrays this limitation
for Legion~\cite{bauer2012legion} applications. Multiple task
threads can issue operations
using distinct communicators, but the polling thread is forced
to iterate over the communicators to process all incoming messages. \changed{Thus, on a single node, the polling thread conflicts with the communicators of the task threads. The polling thread relies
on wildcards, and hence using partitioned operations for this
communication pattern is not straightforward. With endpoints,
on the other hand, the polling thread can use a distinct endpoint,
use wildcards, and satisfy matching requirements.}

%\subsubsection{Mechanism 2: Tags with hints}
\minititle{Mechanism 2: Tags with hints.}
The new Info hints in MPI-4.0 allow domain scientists
to use tags instead of communicators
to express logically parallelism in applications that
do not use certain MPI semantics.

Most \threads{} applications that use
\multiple{} already encode thread IDs into the tags of
their MPI communication to differentiate operations that
target different threads on the same target process
(\eg{}, hypre and Smilei), indicating that
domain scientists intuitively think of tags as a means
of expressing logical parallelism. The approach of using
tags requires the least amount of
changes to existing applications. The changes would
only be in the form of creating a new communicator
with Info hints that relax the MPI semantics
not needed by the application.

\miniminititle{Intricate use of tags.} Even
though tags and communicators have the same
matching constraints, tags can provide more
information. Consider the MPICH library that
features multiple virtual communication interfaces
(VCIs: network communication channels mapping
to distinct network hardware contexts)~\cite{zambre2020learned},
and the hypre library that encodes the IDs of the
sending and receiving threads into the tag along
with other application-related information.
The thread IDs in the tag provide information
about which local and remote VCI to use.
But if MPICH does not know which bits of the tag
encode communication parallelism information,
then hypre is at the mercy of how MPICH hashes
the tags into the multiple VCIs allocated to the
communicator. Achieving the optimal mapping to
VCIs requires hypre to inform MPCIH which bits
encode the sender's thread ID, which bits encode
the receiver's thread ID, and  how to map the bits
to the underlying VCIs. For example, with a one-to-one
mapping, MPICH can use the
sender-thread-bits to map to a VCI on the host
process and the receiver-thread-bits to decide
which VCI to target on the remote process.
Such intricate use of tags requires domain scientists to learn about
the Info hints that are specific to an MPI implementation.

\begin{concern}
	\emph{Concern:} To ensure my code is portable,
	I need to learn about the hints available for each MPI implementation.
\end{concern}

\miniminititle{Lack of portability.}
As just discussed, achieving a high level
of control and flexibility with tags requires a careful
use of implementation-specific Info hints.
It is likely that different MPI implementations
will support tag-based and communicator-based
mechanisms of exposing parallelism in different
ways (VCIs are specific to MPICH; CRIs are specific to Open MPI~\cite{patinyasakdikul2019give}). Since HPC
application developers are geared towards
performance-oriented codes, they are expected
to adopt Info hints to optimally expose logically
parallel communication to an MPI implementation.
Hence, existing MPI mechanisms can result in
reduced portability of codes which is highly undesirable.

\miniminititle{Limited by existing use of tags.} End
users already use MPI tags for
application-related information. Since the number
of bits in a tag is limited, an application may not be
able to encode further parallelism information into
the tag. Encoding parallelism information with
lesser-than-ideal number of bits is bound to hurt
performance.
Although we have not encountered first-hand an
application that faces such a problem, others
have reported running into tag-overflow issues
on prominent applications (\eg{}, SNAP~\cite{snaptag},
Smilei~\cite{smileitag}, and MITgcm~\cite{gcmtag}).
Such reports indicate that applications already use
a large portion of the tag space; encoding
parallelism information into tags exacerbates the
tag-overflow problem.

%\subsubsection{Mechanism 3: User-Visible Endpoints}
\minititle{Mechanism 3: User-Visible Endpoints.}
Given their flexible interface (see \secref{sec:endpoints}),
endpoints combat the various concerns 
associated with communicators and tags to expose
logically parallel point-to-point operations.

\miniminititle{Endpoints are intuitive.}
Endpoints are an easier alternative to express parallelism
even for communication patterns such as
a 3D 27-point stencil. They are more intuitive
to use than communicators because application
developers are already familiar with the semantics
of traditional MPI ranks. Users 
express communication parallelism by simply
communicating between endpoints as they would
do for MPI ranks in \everywhere{} programming. \changed{In
fact, endpoints provide a level of flexibility beyond \everywhere{}:
threads are not bound to an endpoint. In other words,
endpoints do not enforce an association between threads and
the data they work on; a thread can
use any endpoint at any time.}

\miniminititle{Endpoints separate matching and
	parallelism information.}
Unlike existing MPI mechanisms, user-visible
endpoints separate the task of expressing
communication parallelism from the task of
matching operations. Thus, using endpoints is
straightforward even for irregular communication
patterns, such as those of Legion applications (see \figref{fig:legion_comm})
since users can flexibly express parallelism
within a communicator. Endpoints do not suffer from
overloaded definitions of existing MPI objects such
as communicators and tags. Hence, users do not
need to compromise on the application's existing use
of communicators or tags. Furthermore,
the endpoints mechanism directly provides the MPI
library with all the information needed to
optimally map to the underlying network
resources unlike the tag-based mechanism
which requires the application to inform the MPI
library about the specific tag bits that encode
logical parallelism information.

\changed{
\miniminititle{No mismatch in expected mapping to
	network parallelism.} 
By creating an endpoints communicator,
users explicitly inform the MPI library
that the new communicator is
for the purposes of exposing communication parallelism.
This information is baked into the API
unlike the implementation-specific solution of
using hints with communicators or tags.
This incorporation is why endpoints do not suffer from
high resource requirements either. In the example
of executing hypre's 3D 27-point stencil on Bebop,
endpoints require $12.62\times$ fewer VCIs than that
required by communicators~\cite{zambre2021logically}.
}

%\miniminititle{(Almost) No mismatch in expected mapping to
%	network parallelism.}
%User-visible endpoints,
%however, do not completely eliminate the
%potential for a mismatch; domain scientists could create
%more endpoints than the number of underlying
%network resources. In such a scenario, some of 
%the distinct endpoints would contend on the
%underlying network resources and incur overheads
%of thread synchronization. Although
%we have not come across an application that
%would result in such a scenario, we note that even if an
%application's communication pattern requires
%more endpoints than the number of network
%resources, the mismatch problem would hold
%even with other mechanisms.



\miniminititle{Portability.}
The MPI Endpoints effort
encourages standardizing the concept
of endpoints through a new API. With a standardized
interface that provides all the information
that an MPI library needs to optimally map logically
parallel communication to the underlying network
parallelism, applications would be portable across
MPI implementations.

\changed{
\minititle{Mechanism 4: Partitioned Communication.}
Partitioned operations provide the same benefits
as user-visible endpoints on two fronts: first, they do
not overload the definitions of existing MPI objects
and hence minimize the mismatch in expected mapping to
network parallelism; second, they promote
portability of applications across MPI implementations
by their inclusion in the standard. Unlike endpoints that
build on top of existing MPI semantics, however, partitioned
operations introduce new semantics.
How intuitive partitions are to use remains to be seen.
More important though, their semantics have several limitations.
}

\changed{
\miniminititle{Lack of complete independence between threads.}
	The fundamental limitation of partitioned communication
	is that all threads (driving the multiple
	partitions in parallel) share the same message (\ie, the same MPI request).
	So, only a single thread can complete a partitioned
	operation. This means that all threads
	need to synchronize before issuing their
	partition of the next message. Application developers
	could use multiple partitioned operations to reduce
	this synchronization overhead, but they cannot eliminate
	it in a manner like the other two designs can.
    The implicit synchronization requirement of the partitioned interface
	encourages applications to use a fork-join model,
	which has high
	overheads~\cite{baker2012scaling,sahasrabudhe2020improving}, rather than encouraging threads to be asynchronous.
	It is not clear how partitioned
	operations will apply to modern applications where
	threads operate completely independently of each other~\cite{sahasrabudhe2021optimizing,treichler2014realm}.
}

\changed{
\miniminititle{No wildcards.} Partitioned receive operations
cannot use wildcards. Modern event-based runtimes
(\eg{}, Legion~\cite{treichler2014realm} and YGM~\cite{priest2019you}),
however, rely on wildcards in their receiving polling threads. Using
partitioned operations for such runtimes would incur the substantial
overhead of polling for messages from all processes
of the application.
}

\changed{
	\miniminititle{Explosion in API space.} MPI-4.0 currently
	features only a simple send-receive flavor of partitioned
	communication. Expanding the scope of this interface
	to other modes and types of MPI operations requires
	new corresponding APIs (\eg{}, \texttt{MPI\_Pbroadcast\_init}
	for a partitioned broadcast collective). In comparison,
	endpoints require only one new API.
}

==> text/rma_communication.tex <==
\section{Comparison of Designs for RMA Operations}
\label{sec:conversations}

\subsection{RMA}

Given the one-sided nature of RMA
operations with no matching semantics, both existing
MPI mechanisms and user-visible endpoints are
equally straightforward to use, but they have unique concerns.

\miniminititle{Limiting semantics of existing
	MPI mechanisms for atomic operations.}
Using windows to
expose communication parallelism constrains the
parallelism information with MPI's atomicity
semantics. This constraint limits
the user from 
explicitly exposing logically parallel atomic
operations in a single window even when the
application does not need them to be ordered.
In NWChem's block-sparse matrix
multiplication (see \figref{fig:bspmm_comm}),
the \mpiaccum{} operations in a multithreaded
process need to use a single window
to maintain atomicity. Even though the
parallel \mpiaccum{} operations are
independent, users have no
way to explicitly expose this parallelism. The best they
can do is hint the relaxation of MPI's
ordering constraint (\texttt{accumulate\_ordering=none})
and rely on the MPI library's hashing policies
to issue operations on parallel network channels.
These policies, however, are prone
to collisions and will prevent the operations
from mapping to distinct network channels.
With user-visible endpoints, on the other
hand, users can use multiple endpoints
within a single window to expose communication
parallelism \emph{and}
maintain atomicity.

%User-visible endpoints
%decouple the task of exposing parallelism from
%the purposes (\eg{}, atomicity) of existing MPI
%mechanisms.

%=================================================================
\begin{figure*}[!b]
	\vspace{-1.5em}
	\begin{center}
		\includegraphics[width=0.55\textwidth]{pics/bspmm_pattern.pdf}
	\end{center}
		\vspace{-1em}
	\caption{BSPMM: block-sparse matrix multiplication (tensor
		contractions) is the dominant cost in NWChem's simulations~\cite{si2015scaling}.
		The BSPMM uses a \emph{get-compute-update}
		pattern. The matrices are decomposed into tiles and the non-zero
		tiles are evenly distributed between processes. In an \threads{}
		version, threads on all processes collaboratively (using a global
		atomic counter) work on the tile-level multiplication units of
		BSPMM. For each work unit, a thread uses \mpiget{} operations
		to retrieve the tiles it needs, and after the multiplication, it uses
		an \mpiaccum{} operation to update the memory at the target
		location.
	}
	\label{fig:bspmm_comm}
	%\vspace{-1.5em}
\end{figure*}
%=================================================================

\begin{concern}
	\emph{Concern:} Endpoints is a way
	for the MPI library to dump its job on the end user
	a.k.a. domain scientist. I don't know how
	many network endpoints there are. So, how many should I create?
\end{concern}

\miniminititle{Preconceived notions
	about user-visible endpoints.}
A concern that 
came up during our collaboration with
developers of WOMBAT~\cite{mendygral2017wombat}
is the misconception about endpoints being
direct handles to network resources. This
concern holds not just for RMA operations but
also for point-to-point operations.
We learned through our collaborations that this
concern is commonplace in the MPI community.
One explanation for this concern is the usage of the
term "endpoints," which
is typically associated with "network endpoints".
The fact that user-visible endpoints were introduced
for the purposes of utilizing network parallelism
is likely to have exacerbated the misconception.
User-visible endpoints are \emph{not} handles to network
resources, rather they are a means 
to flexibly express communication parallelism. Their usage
is separate from
the MPI library's task to map the exposed
parallelism to the
underlying parallel network resources. The answer
to the question posed in the \emph{concern} is that
applications should create as many endpoints
as there are streams of logically parallel communication.
The MPI library can then funnel the streams of
logically parallel communication on distinct
network hardware contexts depending upon the
availability of network resources.
